Sparse patches adversarial attacks via extrapolating point-wise information

Sparse and patch adversarial attacks were previously shown to be applicable in realistic settings and are considered a security risk to autonomous systems. Sparse adversarial perturbations constitute a setting in which the adversarial perturbations are limited to affecting a relatively small number of points in the input. Patch adversarial attacks denote the setting where the sparse attacks are limited to a given structure, i.e., sparse patches with a given shape and number. However, previous patch adversarial attacks do not simultaneously optimize multiple patches' locations and perturbations. This work suggests a novel approach for sparse patches adversarial attacks via point-wise trimming dense adversarial perturbations. Our approach enables simultaneous optimization of multiple sparse patches' locations and perturbations for any given number and shape. Moreover, our approach is also applicable for standard sparse adversarial attacks, where we show that it significantly improves the state-of-the-art over multiple extensive settings. A reference implementation of the proposed method and the reported experiments is provided at \url{https://github.com/yanemcovsky/SparsePatches.git}

==> vis/fig_IM_CNN.tex <==
\begin{figure}
    \centering
    % \captionsetup{width=\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Imagenet_Inception_v3.pdf}&
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Imagenet_Standard_R50.pdf}&
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Imagenet_Salman2020Do_R50.pdf}
    \end{tabular}
    }
    \caption{
 We compare our method to previous works on the Imagenet dataset $InceptionV3$ model (left), Resnet50 standard model (center), and Resnet50 robust model (right). We report the ASR as a function of $l_0$ over sparse adversarial attacks.
    }
    \label{fig:imagenet_CNN}
\end{figure}


==> vis/fig_attack_vis.tex <==
\begin{figure}
    \centering
    % \captionsetup{width=\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}  
    \toprule
    \textbf{$PGDTrim$ (our)}& 
    \textbf{$CS$}&
    \textbf{$PGD_{L0}$}
    \\
    \midrule
    \multicolumn{3}{c}{True label: \textbf{bird}}
    \\
    % \includegraphics[width=0.2\textwidth]{img/img35_clean_gt_label_bird.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img35_PGDTrimG_gt_label_bird_pred_label_truck.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img35_cs_gt_label_bird_pred_label_truck.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img35_pgdl0_gt_label_bird_pred_label_cat.pdf}
    \\
    Predicted label: \textbf{truck}&
    Predicted label: \textbf{truck}&
    Predicted label: \textbf{cat}
    \\ 
    \midrule
    \multicolumn{3}{c}{True label: \textbf{bird}}
    \\
    % \includegraphics[width=0.2\textwidth]{img/img182_clean_gt_label_bird.pdf}&
    \includegraphics[width=0.2\textwidth] {img/img182_PGDTrimG_gt_label_bird_pred_label_airplane.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img182_cs_gt_label_bird_pred_label_dog.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img182_pgdl0_gt_label_bird_pred_label_automobile.pdf}
    \\
    % True label: \textbf{bird}&
    Predicted label: \textbf{airplane}&
    Predicted label: \textbf{bird}&
    Predicted label: \textbf{automobile}
    \\ 
    \midrule
    \multicolumn{3}{c}{True label: \textbf{deer}}
    \\
    % \includegraphics[width=0.2\textwidth]{img/img227_clean_gt_label_deer.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img227_PGDTrimCB_gt_label_deer_pred_label_cat.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img227_pgdl0_gt_label_deer_pred_label_cat.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img227_cs_gt_label_deer_pred_label_dog.pdf}
    \\
    Predicted label: \textbf{cat}&
    Predicted label: \textbf{cat}&
    Predicted label: \textbf{deer}
    \\ 
    \midrule
    \multicolumn{3}{c}{True label: \textbf{automobile}}
    \\
    % \includegraphics[width=0.2\textwidth]{img/img246_clean_gt_label_automobile.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img246_PGDTrimCB_gt_label_automobile_pred_label_airplane.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img246_cs_gt_label_automobile_pred_label_truck.pdf}&
    \includegraphics[width=0.2\textwidth]{img/img246_pgdl0_gt_label_automobile_pred_label_airplane.pdf}
    \\
    Predicted label: \textbf{airplane}&
    Predicted label: \textbf{automobile}&
    Predicted label: \textbf{airplane}
    \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    Visualization of sparse adversarial attacks on CIFAR10 standard Wide-ResNet28-10, for attacks bounded to $\epsilon_0=8$. We present the produced adversarial inputs, and the labels predicted for each compared to the true label.
    }
    \label{fig:attack_vis}
\end{figure}


==> vis/fig_cifar10_R18.tex <==
\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc}  
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Cifar10_Resnet18.pdf}&
    \includegraphics[width=\textwidth]{fig/best_patch_attacks_success_l_inf_1_Cifar10_Resnet18.pdf}
    \end{tabular}
    }
    \caption{
We compare our method to previous sparse attack works(left) and with various patch sizes (right) on the CIFAR10 dataset ResNet-18 standard model. We report the ASR as a function of $l_0$ for all attacks.
    }
    \label{fig:cifar10_R18}
\end{figure}


==> vis/fig_cifar10_RWR28_10.tex <==
\begin{figure}
    \centering
    % \captionsetup{width=\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc}  
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Cifar10_Wang2023Better_WRN-28-10.pdf}&
    \includegraphics[width=\textwidth]{fig/best_patch_attacks_success_l_inf_1_Cifar10_Wang2023Better_WRN-28-10.pdf}
    \end{tabular}
    }
    \caption{
We compare our method to previous sparse attack works(left) and with various patch sizes (right) on the CIFAR10 dataset Wide-ResNet28-10 robust model. We report the ASR as a function of $l_0$ for all attacks.
    }
    \label{fig:cifar10_RWR}
\end{figure}


==> vis/fig_cifar10_SWR28_10.tex <==
\begin{figure}
    \centering
    % \captionsetup{width=\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc}  
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Cifar10_Standard.pdf}&
    \includegraphics[width=\textwidth]{fig/best_patch_attacks_success_l_inf_1_Cifar10_Standard.pdf}
    \end{tabular}
    }
    \caption{
We compare our method to previous sparse attack works(left) and with various patch sizes (right) on the CIFAR10 dataset Wide-ResNet28-10 standard model. We report the ASR as a function of $l_0$ for all attacks.
    }
    \label{fig:cifar10_SWR}
\end{figure}


==> vis/fig_cifar10_WR28_10.tex <==
\begin{figure}
    \centering
    % \captionsetup{width=\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc}  
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Cifar10_Standard.pdf}&
    \includegraphics[width=\textwidth]{fig/best_sparse_attacks_success_l_inf_1_Cifar10_Wang2023Better_WRN-28-10.pdf}
    \end{tabular}
    }
    \caption{
 We compare our method to previous works on the CIFAR10 dataset Wide-ResNet28-10 standard model (left) and robust model (right). We report the ASR as a function of $l_0$ over all adversarial attacks.
    }
    \label{fig:cifar10_WR}
\end{figure}


==> vis/fig_trim_vis2.tex <==
\begin{figure*}
 \centering
    \includegraphics[width=\linewidth]{img/fig_trim.pdf}
 \caption{
    Flowchart of our sparse adversarial attack's trim process on Imagenet $InceptionV3$ model, for attacks bounded to $\epsilon_0=299$. We present the adversarial inputs produced for distinct $\epsilon_0$ bounds during the process and the predicted label for each, compared to the true label\yaniv{add another figure with patches}.
 }
\label{fig:trim_vis}
\end{figure*}


==> vis/table_cifar10.tex <==


\begin{table}
    \centering
    \caption{
    Comparison of sparse adversarial attacks on CIFAR10 dataset ResNet-18, standard Wide-ResNet28-10, and robust Wide-ResNet28-10 models. For each model and attack, we report the clean accuracy and the ASR under each of the considered bounds.
  }
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccc}  
        \toprule
        \textbf{Attack}&\textbf{ ASR$_{\epsilon_{0}=8}^{\epsilon_{\infty}=1}$}&\textbf{ASR$_{\epsilon_{0}=32}^{\epsilon_{\infty}=1}$}&\textbf{ASR$_{\epsilon_{0}=8}^{\epsilon_{\infty}=\nicefrac{8}{255}}$}&\textbf{ASR$_{\epsilon_{0}=32}^{\epsilon_{\infty}=\nicefrac{8}{255}}$} \\ 
        \midrule
        % \multicolumn{5}{c}{\textbf{Model}: ResNet-18, \textbf{Clean accuracy}:$94.22\%$}  \\
        \multicolumn{3}{c}{\textbf{Model}: ResNet-18} & \multicolumn{2}{c}{\textbf{Clean accuracy}: $94.22\%$}  \\
        \midrule
        $PGDTrim$  & $\mathbf{96.64}$ &$\mathbf{100}$ & $\mathbf{13.16}$ & $\mathbf{55.75}$ \\
        $CS$       & $94.63$          &$98.29$        & $12.48$          & $36.49$  \\
        $PGD_{L0}$ & $77.58$          &$\mathbf{100}$ & $11.02$          & $43.56$  \\
        \midrule
        % \multicolumn{5}{c}{\textbf{Model}: Wide-ResNet28-10, \textbf{Clean accuracy}:$94.78\%$}  \\
        \multicolumn{3}{c}{\textbf{Model}: Wide-ResNet28-10} & \multicolumn{2}{c}{\textbf{Clean accuracy}: $94.78\%$}  \\
        \midrule
        $PGDTrim$  & $\mathbf{93.57}$ &$\mathbf{100}$ & $\mathbf{14.89}$ & $\mathbf{61.16}$ \\
        $CS$       & $87.80$          &$94.24$        & $14.73$          & $36.80$  \\
        $PGD_{L0}$ & $72.76$          &$99.42$        & $11.82$          & $42.67$  \\
        \midrule
        % \multicolumn{5}{c}{\textbf{Model}: robust Wide-ResNet28-10, \textbf{Clean accuracy}:$94.44\%$}  \\
        \multicolumn{3}{c}{\textbf{Model}: robust Wide-ResNet28-10} & \multicolumn{2}{c}{\textbf{Clean accuracy}: $94.44\%$}  \\
        \midrule
        $PGDTrim$  & $50.01$          &$\mathbf{92.41}$ & $\mathbf{3.41}$ & $6.15$ \\
        $CS$       & $\mathbf{54.29}$ &$67.76$          & $3.28$          & $5.43$  \\
        $PGD_{L0}$ & $32.84$          &$84.47$          & $3.39$          & $\mathbf{6.20}$  \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:CIFAR_10}
\end{table}


==> vis/table_imagenet.tex <==


\begin{table}
    \centering
    \caption{
        Comparison of sparse adversarial attacks on ImageNet dataset. We report the ASR of each attack on each model over several $\epsilon_{0}$ bounds.
  }
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccccc}  
        \toprule
        \textbf{Attack}&\textbf{Model}&\textbf{input size (N)}&\textbf{ ASR$_{\epsilon_{0}=8}$}&\textbf{ASR$_{\epsilon_{0}=32}$}&\textbf{ASR$_{\epsilon_{0}=\sqrt{N}}$} \\ 
        % \midrule
        % % \multicolumn{5}{c}{\textbf{Model}: InceptionV3, \textbf{Clean accuracy}:$77.4\%$}  \\
        % \multicolumn{3}{c}{\textbf{Model}: $InceptionV3$} & \multicolumn{2}{c}{\textbf{Clean accuracy}: $77.4\%$}  \\
        \midrule
        $PGDTrim$ &  $InceptionV3$ & $299^2$  & $\mathbf{00.00}$ &$\mathbf{00.00}$ & $\mathbf{00.00}$ \\
        $PGD_{L0}$ & $InceptionV3$ & $299^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $GF$ &       $InceptionV3$ & $299^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $SF$ &       $InceptionV3$ & $299^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $Homotopy$ & $InceptionV3$ & $299^2$  & $00.00$          &$00.00$          & $00.00$          \\
        \midrule
        $PGDTrim$ &  Standard $Resnet50$ & $224^2$  & $\mathbf{00.00}$ &$\mathbf{00.00}$ & $\mathbf{00.00}$ \\
        $PGD_{L0}$ & Standard $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $GF$ &       Standard $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $SF$ &       Standard $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $Homotopy$ & Standard $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        \midrule
        $PGDTrim$ &  Robust $Resnet50$ & $224^2$  & $\mathbf{00.00}$ &$\mathbf{00.00}$ & $\mathbf{00.00}$ \\
        $PGD_{L0}$ & Robust $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $GF$ &       Robust $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $SF$ &       Robust $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $Homotopy$ & Robust $Resnet50$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        \midrule
        $PGDTrim$ &  $Swin-B$ & $224^2$  & $\mathbf{00.00}$ &$\mathbf{00.00}$ & $\mathbf{00.00}$ \\
        $PGD_{L0}$ & $Swin-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $GF$ &       $Swin-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $SF$ &       $Swin-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $Homotopy$ & $Swin-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        \midrule
        $PGDTrim$ &  $ConvNeXt-B$ & $224^2$  & $\mathbf{00.00}$ &$\mathbf{00.00}$ & $\mathbf{00.00}$ \\
        $PGD_{L0}$ & $ConvNeXt-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $GF$ &       $ConvNeXt-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $SF$ &       $ConvNeXt-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\
        $Homotopy$ & $ConvNeXt-B$ & $224^2$  & $00.00$          &$00.00$          & $00.00$          \\

        \bottomrule
    \end{tabular}
    }
    \label{tab:imagenet}
\end{table}

